ParGeo: A Library for Parallel Computational Geometry

This paper presents ParGeo, a multicore library for computational geometry. ParGeo contains modules for fundamental tasks including $k$d-tree based spatial search, spatial graph generation, and algorithms in computational geometry. We focus on three new algorithmic contributions provided in the library. First, we present a new parallel convex hull algorithm based on a reservation technique to enable parallel modifications to the hull. We also provide the first parallel implementations of the randomized incremental convex hull algorithm as well as a divide-and-conquer convex hull algorithm in $\mathbb{R}^3$. Second, for the smallest enclosing ball problem, we propose a new sampling-based algorithm to quickly reduce the size of the data set. We also provide the first parallel implementation of Welzl's classic algorithm for smallest enclosing ball. Third, we present the BDL-tree, a parallel batch-dynamic $k$d-tree that allows for efficient parallel updates and $k$-NN queries over dynamically changing point sets. BDL-trees consist of a log-structured set of $k$d-trees which can be used to efficiently insert, delete, and query batches of points in parallel. On 36 cores with two-way hyper-threading, our fastest convex hull algorithm achieves up to 44.7x self-relative parallel speedup and up to 559x speedup against the best existing sequential implementation. Our smallest enclosing ball algorithm using our sampling-based algorithm achieves up to 27.1x self-relative parallel speedup and up to 178x speedup against the best existing sequential implementation. Our implementation of the BDL-tree achieves self-relative parallel speedup of up to 46.1x. Across all of the algorithms in ParGeo, we achieve self-relative parallel speedup of 8.1--46.61x.

==> batch-kdtree/data/construction_100-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &     B1 &     B2 &      BDL &            B1 &           B2 &             BDL \\
\midrule
2D-U-10M &  20.6s &  16.3s &  14.4s &  0.5s (40.0x) &  3.7s (4.5x) &  0.4s (34.5x) \\
2D-V-10M &  20.5s &  16.2s &  14.2s &  0.5s (40.3x) &  3.6s (4.5x) &  0.4s (34.8x) \\
5D-U-10M &  23.3s &  20.8s &  16.3s &  0.7s (35.2x) &  4.8s (4.3x) &  0.5s (30.3x) \\
5D-V-10M &  22.8s &  20.2s &  15.8s &  0.7s (34.9x) &  4.6s (4.4x) &  0.5s (29.2x) \\
7D-U-10M &  27.0s &  24.0s &  17.1s &  0.8s (33.0x) &  5.4s (4.4x) &  0.6s (27.5x) \\
7D-V-10M &  26.2s &  23.2s &  16.5s &  0.8s (33.5x) &  5.3s (4.4x) &  0.6s (26.6x) \\
10D-H-1M &   1.5s &   1.5s &   2.8s &  0.1s (23.7x) &  0.5s (3.4x) &  0.1s (23.8x) \\
16D-C-4M &  13.5s &  14.5s &  11.0s &  0.5s (25.2x) &  3.8s (3.8x) &  0.5s (20.4x) \\
3D-C-321M & -- & -- & -- & -- & -- & 20.4s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/construction_100-spatial.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &     B1 &    B2 &      BDL &            B1 &           B2 &             BDL \\
\midrule
2D-U-10M &  10.7s &  2.3s &   5.3s &  0.5s (23.8x) &  1.6s (1.4x) &  0.4s (13.5x) \\
2D-V-10M &  10.9s &  2.5s &   5.5s &  0.5s (22.8x) &  1.7s (1.5x) &  0.4s (13.5x) \\
5D-U-10M &  13.7s &  3.4s &  6.7s &  0.8s (18.0x) &  2.3s (1.5x) &  0.6s (10.7x) \\
5D-V-10M &  14.4s &  4.0s &  7.1s &  0.8s (17.4x) &  2.6s (1.5x) &  0.7s (10.3x) \\
7D-U-10M &  16.8s &  4.4s &  7.1s &  1.0s (17.2x) &  2.9s (1.5x) &  0.8s (9.3x) \\
7D-V-10M &  17.3s &  5.2s &  8.3s &  1.0s (16.9x) &  3.3s (1.6x) &  0.9s (9.2x) \\
10D-H-1M &   1.4s &  0.8s &   3.2s &  0.1s (11.0x) &  0.5s (1.6x) &  0.2s (15.9x) \\
16D-C-4M &  10.0s &  5.3s &   7.3s &  0.7s (14.0x) &  3.0s (1.8x) &  0.7s (10.2x) \\
3D-C-321M & -- & -- & -- & -- & -- & 20.8s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/construction_100.tex <==
\begin{tabular}{lllllllll}
\toprule
{} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{36h} \\
{} & balanced-object & balanced-spatial & logtree-object & logtree-spatial & balanced-object & balanced-spatial & logtree-object & logtree-spatial \\
\midrule
2D-uniform-10M   &           20.6s &            10.7s &          18.4s &            9.5s &    0.5s (40.0x) &     0.5s (23.8x) &   0.5s (35.4x) &    0.5s (18.9x) \\
2D-visualvar-10M &           20.5s &            10.9s &          18.3s &            9.6s &    0.5s (40.3x) &     0.5s (22.8x) &   0.5s (35.2x) &    0.5s (19.0x) \\
5D-uniform-10M   &           23.3s &            13.7s &          20.6s &           12.1s &    0.7s (35.2x) &     0.8s (18.0x) &   0.6s (32.4x) &    0.8s (15.3x) \\
5D-visualvar-10M &           22.8s &            14.4s &          20.1s &           12.6s &    0.7s (34.9x) &     0.8s (17.4x) &   0.6s (32.1x) &    0.8s (15.0x) \\
7D-uniform-10M   &           27.0s &            16.8s &          23.7s &           13.7s &    0.8s (33.0x) &     1.0s (17.2x) &   0.8s (29.7x) &    1.0s (14.2x) \\
7D-visualvar-10M &           26.2s &            17.3s &          23.1s &           14.3s &    0.8s (33.5x) &     1.0s (16.9x) &   0.8s (29.2x) &    1.0s (14.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/construction_100_old.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} & balanced & logtree &      balanced &       logtree \\
\midrule
2D-uniform-10M-object    &    20.6s &   18.4s &  0.5s (40.0x) &  0.5s (35.4x) \\
2D-uniform-10M-spatial   &    10.7s &    9.5s &  0.5s (23.8x) &  0.5s (18.9x) \\
2D-visualvar-10M-object  &    20.5s &   18.3s &  0.5s (40.3x) &  0.5s (35.2x) \\
2D-visualvar-10M-spatial &    10.9s &    9.6s &  0.5s (22.8x) &  0.5s (19.0x) \\
5D-uniform-10M-object    &    23.3s &   20.6s &  0.7s (35.2x) &  0.6s (32.4x) \\
5D-uniform-10M-spatial   &    13.7s &   12.1s &  0.8s (18.0x) &  0.8s (15.3x) \\
5D-visualvar-10M-object  &    22.8s &   20.1s &  0.7s (34.9x) &  0.6s (32.1x) \\
5D-visualvar-10M-spatial &    14.4s &   12.6s &  0.8s (17.4x) &  0.8s (15.0x) \\
7D-uniform-10M-object    &    27.0s &   23.7s &  0.8s (33.0x) &  0.8s (29.7x) \\
7D-uniform-10M-spatial   &    16.8s &   13.7s &  1.0s (17.2x) &  1.0s (14.2x) \\
7D-visualvar-10M-object  &    26.2s &   23.1s &  0.8s (33.5x) &  0.8s (29.2x) \\
7D-visualvar-10M-spatial &    17.3s &   14.3s &  1.0s (16.9x) &  1.0s (14.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/delete_10.tex <==
\begin{tabular}{lllllllll}
\toprule
{} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{36h} \\
{} & balanced-object & balanced-spatial & logtree-object & logtree-spatial & balanced-object & balanced-spatial & logtree-object & logtree-spatial \\
\midrule
2D-uniform-10M   &          114.0s &            70.2s &          29.2s &           30.2s &    2.7s (43.0x) &     1.8s (38.8x) &   0.9s (33.0x) &    1.1s (26.3x) \\
2D-visualvar-10M &          114.2s &            71.7s &          29.0s &           30.7s &    2.7s (43.0x) &     2.0s (36.0x) &   0.9s (33.1x) &    1.2s (25.4x) \\
5D-uniform-10M   &          130.2s &            82.9s &          40.1s &           29.2s &    3.5s (37.2x) &     2.9s (28.9x) &   1.4s (28.1x) &    1.2s (23.9x) \\
5D-visualvar-10M &          127.0s &            85.9s &          39.3s &           29.6s &    3.5s (36.8x) &     3.4s (25.4x) &   1.4s (27.8x) &    1.3s (22.2x) \\
7D-uniform-10M   &          146.7s &            97.1s &          37.3s &           38.2s &    4.1s (36.0x) &     3.6s (27.1x) &   1.4s (27.0x) &    1.8s (21.4x) \\
7D-visualvar-10M &          144.4s &           100.8s &          36.9s &           38.3s &    4.1s (35.6x) &     4.2s (24.0x) &   1.4s (27.2x) &    1.8s (20.9x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/delete_10_old.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} & balanced & logtree &      balanced &       logtree \\
\midrule
2D-uniform-10M-object    &   114.0s &   29.2s &  2.7s (43.0x) &  0.9s (33.0x) \\
2D-uniform-10M-spatial   &    70.2s &   30.2s &  1.8s (38.8x) &  1.1s (26.3x) \\
2D-visualvar-10M-object  &   114.2s &   29.0s &  2.7s (43.0x) &  0.9s (33.1x) \\
2D-visualvar-10M-spatial &    71.7s &   30.7s &  2.0s (36.0x) &  1.2s (25.4x) \\
5D-uniform-10M-object    &   130.2s &   40.1s &  3.5s (37.2x) &  1.4s (28.1x) \\
5D-uniform-10M-spatial   &    82.9s &   29.2s &  2.9s (28.9x) &  1.2s (23.9x) \\
5D-visualvar-10M-object  &   127.0s &   39.3s &  3.5s (36.8x) &  1.4s (27.8x) \\
5D-visualvar-10M-spatial &    85.9s &   29.6s &  3.4s (25.4x) &  1.3s (22.2x) \\
7D-uniform-10M-object    &   146.7s &   37.3s &  4.1s (36.0x) &  1.4s (27.0x) \\
7D-uniform-10M-spatial   &    97.1s &   38.2s &  3.6s (27.1x) &  1.8s (21.4x) \\
7D-visualvar-10M-object  &   144.4s &   36.9s &  4.1s (35.6x) &  1.4s (27.2x) \\
7D-visualvar-10M-spatial &   100.8s &   38.3s &  4.2s (24.0x) &  1.8s (20.9x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/insert_10.tex <==
\begin{tabular}{lllllllll}
\toprule
{} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{36h} \\
{} & balanced-object & balanced-spatial & logtree-object & logtree-spatial & balanced-object & balanced-spatial & logtree-object & logtree-spatial \\
\midrule
2D-uniform-10M   &           86.1s &            32.5s &          33.1s &           13.6s &    2.2s (39.5x) &     1.2s (26.1x) &   0.9s (35.0x) &    0.8s (16.5x) \\
2D-visualvar-10M &           86.1s &            33.9s &          32.8s &           14.2s &    2.2s (39.6x) &     1.4s (24.0x) &   0.9s (34.6x) &    0.9s (16.1x) \\
5D-uniform-10M   &           97.9s &            40.7s &          39.1s &           19.0s &    2.9s (33.6x) &     2.3s (17.5x) &   1.3s (30.8x) &    1.4s (13.4x) \\
5D-visualvar-10M &           94.5s &            44.5s &          38.0s &           20.0s &    2.8s (33.2x) &     2.8s (15.6x) &   1.3s (30.2x) &    1.6s (12.9x) \\
7D-uniform-10M   &          109.7s &            48.1s &          44.0s &           22.0s &    3.5s (31.1x) &     3.1s (15.6x) &   1.5s (28.9x) &    1.8s (12.4x) \\
7D-visualvar-10M &          106.1s &            52.6s &          42.7s &           23.2s &    3.5s (30.7x) &     3.7s (14.4x) &   1.5s (27.8x) &    1.9s (12.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_combined_old/insert_10_old.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} & balanced & logtree &      balanced &       logtree \\
\midrule
2D-uniform-10M-object    &    86.1s &   33.1s &  2.2s (39.5x) &  0.9s (35.0x) \\
2D-uniform-10M-spatial   &    32.5s &   13.6s &  1.2s (26.1x) &  0.8s (16.5x) \\
2D-visualvar-10M-object  &    86.1s &   32.8s &  2.2s (39.6x) &  0.9s (34.6x) \\
2D-visualvar-10M-spatial &    33.9s &   14.2s &  1.4s (24.0x) &  0.9s (16.1x) \\
5D-uniform-10M-object    &    97.9s &   39.1s &  2.9s (33.6x) &  1.3s (30.8x) \\
5D-uniform-10M-spatial   &    40.7s &   19.0s &  2.3s (17.5x) &  1.4s (13.4x) \\
5D-visualvar-10M-object  &    94.5s &   38.0s &  2.8s (33.2x) &  1.3s (30.2x) \\
5D-visualvar-10M-spatial &    44.5s &   20.0s &  2.8s (15.6x) &  1.6s (12.9x) \\
7D-uniform-10M-object    &   109.7s &   44.0s &  3.5s (31.1x) &  1.5s (28.9x) \\
7D-uniform-10M-spatial   &    48.1s &   22.0s &  3.1s (15.6x) &  1.8s (12.4x) \\
7D-visualvar-10M-object  &   106.1s &   42.7s &  3.5s (30.7x) &  1.5s (27.8x) \\
7D-visualvar-10M-spatial &    52.6s &   23.2s &  3.7s (14.4x) &  1.9s (12.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/construction_100-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &     B2 &    B1 &      L &            B2 &           B1 &             L \\
\midrule
2D-U-10M &  20.6s &  2.8s &  18.4s &  0.5s (40.0x) &  3.5s (0.8x) &  0.5s (35.4x) \\
2D-V-10M &  20.5s &  2.8s &  18.3s &  0.5s (40.3x) &  3.5s (0.8x) &  0.5s (35.2x) \\
5D-U-10M &  23.3s &  3.5s &  20.6s &  0.7s (35.2x) &  4.3s (0.8x) &  0.6s (32.4x) \\
5D-V-10M &  22.8s &  3.3s &  20.1s &  0.7s (34.9x) &  4.1s (0.8x) &  0.6s (32.1x) \\
7D-U-10M &  27.0s &  4.0s &  23.7s &  0.8s (33.0x) &  4.9s (0.8x) &  0.8s (29.7x) \\
7D-V-10M &  26.2s &  4.0s &  23.1s &  0.8s (33.5x) &  4.9s (0.8x) &  0.8s (29.2x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/construction_100-spatial.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} &     B2 &      L &            B2 &             L \\
\midrule
2D-U-10M &  10.7s &   9.5s &  0.5s (23.8x) &  0.5s (18.9x) \\
2D-V-10M &  10.9s &   9.6s &  0.5s (22.8x) &  0.5s (19.0x) \\
5D-U-10M &  13.7s &  12.1s &  0.8s (18.0x) &  0.8s (15.3x) \\
5D-V-10M &  14.4s &  12.6s &  0.8s (17.4x) &  0.8s (15.0x) \\
7D-U-10M &  16.8s &  13.7s &  1.0s (17.2x) &  1.0s (14.2x) \\
7D-V-10M &  17.3s &  14.3s &  1.0s (16.9x) &  1.0s (14.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/delete_10-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &      B2 &    B1 &      L &            B2 &           B1 &             L \\
\midrule
2D-U-10M &  114.0s &  0.6s &  29.2s &  2.7s (43.0x) &  0.1s (5.4x) &  0.9s (33.0x) \\
2D-V-10M &  114.2s &  0.6s &  29.0s &  2.7s (43.0x) &  0.1s (5.4x) &  0.9s (33.1x) \\
5D-U-10M &  130.2s &  0.7s &  40.1s &  3.5s (37.2x) &  0.2s (3.2x) &  1.4s (28.1x) \\
5D-V-10M &  127.0s &  0.7s &  39.3s &  3.5s (36.8x) &  0.2s (3.2x) &  1.4s (27.8x) \\
7D-U-10M &  146.7s &  0.9s &  37.3s &  4.1s (36.0x) &  0.3s (3.0x) &  1.4s (27.0x) \\
7D-V-10M &  144.4s &  0.9s &  36.9s &  4.1s (35.6x) &  0.3s (3.0x) &  1.4s (27.2x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/delete_10-spatial.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} &      B2 &      L &            B2 &             L \\
\midrule
2D-U-10M &   70.2s &  30.2s &  1.8s (38.8x) &  1.1s (26.3x) \\
2D-V-10M &   71.7s &  30.7s &  2.0s (36.0x) &  1.2s (25.4x) \\
5D-U-10M &   82.9s &  29.2s &  2.9s (28.9x) &  1.2s (23.9x) \\
5D-V-10M &   85.9s &  29.6s &  3.4s (25.4x) &  1.3s (22.2x) \\
7D-U-10M &   97.1s &  38.2s &  3.6s (27.1x) &  1.8s (21.4x) \\
7D-V-10M &  100.8s &  38.3s &  4.2s (24.0x) &  1.8s (20.9x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/insert_10-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &      B2 &    B1 &      L &            B2 &           B1 &             L \\
\midrule
2D-U-10M &   86.1s &  4.7s &  33.1s &  2.2s (39.5x) &  0.5s (8.6x) &  0.9s (35.0x) \\
2D-V-10M &   86.1s &  4.7s &  32.8s &  2.2s (39.6x) &  0.5s (8.6x) &  0.9s (34.6x) \\
5D-U-10M &   97.9s &  5.7s &  39.1s &  2.9s (33.6x) &  0.7s (7.6x) &  1.3s (30.8x) \\
5D-V-10M &   94.5s &  5.7s &  38.0s &  2.8s (33.2x) &  0.7s (7.7x) &  1.3s (30.2x) \\
7D-U-10M &  109.7s &  6.4s &  44.0s &  3.5s (31.1x) &  0.9s (7.4x) &  1.5s (28.9x) \\
7D-V-10M &  106.1s &  6.3s &  42.7s &  3.5s (30.7x) &  0.9s (7.4x) &  1.5s (27.8x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/insert_10-spatial.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} &     B2 &      L &            B2 &             L \\
\midrule
2D-U-10M &  32.5s &  13.6s &  1.2s (26.1x) &  0.8s (16.5x) \\
2D-V-10M &  33.9s &  14.2s &  1.4s (24.0x) &  0.9s (16.1x) \\
5D-U-10M &  40.7s &  19.0s &  2.3s (17.5x) &  1.4s (13.4x) \\
5D-V-10M &  44.5s &  20.0s &  2.8s (15.6x) &  1.6s (12.9x) \\
7D-U-10M &  48.1s &  22.0s &  3.1s (15.6x) &  1.8s (12.4x) \\
7D-V-10M &  52.6s &  23.2s &  3.7s (14.4x) &  1.9s (12.1x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/knn_consolidated-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &       B2 &       B1 &        L &             B2 &             B1 &              L \\
\midrule
2D-U-10M &    34.9s &    13.6s &    95.0s &   0.6s (57.2x) &   0.3s (40.8x) &   2.1s (46.2x) \\
2D-V-10M &    37.2s &    14.6s &   100.5s &   0.7s (57.0x) &   0.4s (40.9x) &   2.1s (47.1x) \\
5D-U-10M &   302.3s &   200.1s &   591.6s &   6.3s (47.6x) &   3.9s (51.6x) &  14.1s (41.9x) \\
5D-V-10M &   109.5s &    71.1s &   229.5s &   2.1s (51.1x) &   1.3s (53.0x) &   4.8s (47.4x) \\
7D-U-10M &  1520.0s &  1407.6s &  2740.7s &  44.3s (34.3x) &  38.8s (36.3x) &  83.3s (32.9x) \\
7D-V-10M &   133.6s &    97.0s &   307.0s &   2.8s (48.1x) &   1.9s (50.9x) &   6.7s (46.0x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/data_dyn_1/knn_consolidated-spatial.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} &       B2 &        L &             B2 &              L \\
\midrule
2D-U-10M &    33.6s &    97.2s &   0.6s (55.6x) &   2.0s (48.0x) \\
2D-V-10M &    35.7s &   104.6s &   0.6s (56.8x) &   2.1s (48.9x) \\
5D-U-10M &   348.8s &   801.0s &   6.7s (52.2x) &  15.2s (52.8x) \\
5D-V-10M &   103.1s &   244.5s &   2.0s (52.8x) &   4.8s (51.1x) \\
7D-U-10M &  2142.0s &  4255.1s &  45.5s (47.1x) &  85.1s (50.0x) \\
7D-V-10M &   116.9s &   303.1s &   2.3s (50.5x) &   6.0s (50.2x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/datasets.tex <==
\begin{tabular}{lll}
\toprule
Description          & Size (\# points) & Dimension \\ \midrule
Uniform Distribution & 10M              & 2         \\
Uniform Distribution & 10M              & 5         \\
Uniform Distribution & 10M              & 7         \\
Visual Data          & 10M              & 2         \\
Visual Data          & 10M              & 5         \\
Visual Data          & 10M              & 7         \\
HT (Real-World)\todo{describe}      & 1M               & 10        \\
CHEM (Real-World)\todo{describe}    & 4M               & 16        \\
\bottomrule
\end{tabular}

==> batch-kdtree/data/delete_10-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &      B1 &    B2 &      BDL &            B1 &            B2 &             BDL \\
\midrule
2D-U-10M &  114.0s &  1.1s &  29.2s &  2.7s (43.0x) &  0.1s (10.4x) &  0.9s (33.0x) \\
2D-V-10M &  114.2s &  1.1s &  29.0s &  2.7s (43.0x) &  0.1s (10.5x) &  0.9s (33.1x) \\
5D-U-10M &  130.2s &  2.2s &  40.1s &  3.5s (37.2x) &   0.2s (9.1x) &  1.4s (28.1x) \\
5D-V-10M &  127.0s &  2.2s &  39.3s &  3.5s (36.8x) &   0.2s (9.1x) &  1.4s (27.8x) \\
7D-U-10M &  146.7s &  3.0s &  37.3s &  4.1s (36.0x) &   0.3s (8.9x) &  1.4s (27.0x) \\
7D-V-10M &  144.4s &  3.0s &  36.9s &  4.1s (35.6x) &   0.3s (8.9x) &  1.4s (27.2x) \\
10D-H-1M &   24.7s &  0.2s &  21.9s &  1.0s (24.7x) &   0.0s (5.6x) &  0.8s (28.5x) \\
16D-C-4M &   74.8s &  2.9s &  33.1s &  2.7s (27.4x) &   0.3s (8.6x) &  1.4s (23.6x) \\
3D-C-321M & -- & -- & -- & -- & -- & 17.3s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/delete_10-spatial.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &      B1 &    B2 &      BDL &            B1 &            B2 &             BDL \\
\midrule
2D-U-10M &   70.2s &  1.3s &  30.2s &  1.8s (38.8x) &  0.1s (11.8x) &  1.1s (26.3x) \\
2D-V-10M &   71.7s &  1.5s &  30.7s &  2.0s (36.0x) &  0.1s (10.7x) &  1.2s (25.4x) \\
5D-U-10M &   82.9s &  2.3s &  29.2s &  2.9s (28.9x) &   0.2s (9.6x) &  1.2s (23.9x) \\
5D-V-10M &   85.9s &  2.9s &  29.6s &  3.4s (25.4x) &   0.3s (9.0x) &  1.3s (22.2x) \\
7D-U-10M &   97.1s &  3.2s &  38.2s &  3.6s (27.1x) &   0.3s (9.4x) &  1.8s (21.4x) \\
7D-V-10M &  100.8s &  3.9s &  38.3s &  4.2s (24.0x) &   0.4s (8.8x) &  1.8s (20.9x) \\
10D-H-1M &   27.6s &  0.4s &  22.1s &  1.1s (25.1x) &   0.1s (4.8x) &  0.8s (26.2x) \\
16D-C-4M &   60.5s &  4.0s &  32.5s &  3.3s (18.3x) &   0.5s (8.8x) &  1.7s (19.5x) \\
3D-C-321M & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/format.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\

==> batch-kdtree/data/insert_10-object.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &      B1 &    B2 &     BDL &            B1 &            B2 &             BDL \\
\midrule
2D-U-10M &   86.1s &  5.9s &  24.8s &  2.2s (39.5x) &  0.6s (10.1x) &  0.7s (35.4x) \\
2D-V-10M &   86.1s &  5.9s &  24.4s &  2.2s (39.6x) &  0.6s (10.2x) &  0.7s (35.5x) \\
5D-U-10M &   97.9s &  7.6s &  29.2s &  2.9s (33.6x) &   0.9s (8.7x) &  1.0s (30.3x) \\
5D-V-10M &   94.5s &  7.5s &  28.1s &  2.8s (33.2x) &   0.9s (8.8x) &  1.0s (29.3x) \\
7D-U-10M &  109.7s &  8.8s &  33.0s &  3.5s (31.1x) &   1.1s (8.1x) &  1.2s (26.9x) \\
7D-V-10M &  106.1s &  8.7s &  31.7s &  3.5s (30.7x) &   1.1s (8.2x) &  1.2s (25.6x) \\
10D-H-1M &    7.9s &  0.7s &   1.7s &  0.4s (22.1x) &   0.1s (5.7x) &  0.1s (16.3x) \\
16D-C-4M &   66.2s &  5.5s &  21.1s &  3.0s (22.2x) &   0.9s (6.4x) &  1.1s (18.3x) \\
3D-C-321M & -- & -- & -- & -- & -- & 20.7s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/insert_10-spatial.tex <==
\begin{tabular}{@{}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{\hskip5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &     B1 &    B2 &      BDL &            B1 &            B2 &             BDL \\
\midrule
2D-U-10M &  32.5s &  4.9s &  5.2s &  1.2s (26.1x) &  0.4s (11.9x) &  0.6s (9.2x) \\
2D-V-10M &  33.9s &  5.0s &  5.8s &  1.4s (24.0x) &  0.5s (10.2x) &  0.6s (9.2x) \\
5D-U-10M &  40.7s &  6.1s &  8.8s &  2.3s (17.5x) &   0.7s (9.4x) &  1.1s (8.1x) \\
5D-V-10M &  44.5s &  6.7s &  10.0s &  2.8s (15.6x) &   0.8s (8.0x) &  1.2s (8.0x) \\
7D-U-10M &  48.1s &  7.0s &  11.2s &  3.1s (15.6x) &   0.8s (8.5x) &  1.5s (7.4x) \\
7D-V-10M &  52.6s &  7.6s &  12.5s &  3.7s (14.4x) &   1.0s (7.8x) &  1.6s (7.6x) \\
10D-H-1M &   6.3s &  0.9s &   1.3s &  0.6s (10.2x) &   0.2s (3.8x) &   0.2s (6.6x) \\
16D-C-4M &  42.9s &  6.0s &  12.9s &  3.6s (11.8x) &   1.0s (5.9x) &  1.5s (8.5x) \\
3D-C-321M & -- & -- & -- & -- & -- & 15.7s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/knn_DKNN_nonatomic_5-object.tex <==
\begin{tabular}{lllll}
\toprule
{} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{36h} \\
{} & BDL-object & BDL-spatial &        BDL-object &      BDL-spatial \\
\midrule
2D-U-10M &    53.3s &     47.0s &    4.3s (12.3x) &   2.7s (17.2x) \\
2D-V-10M &    56.0s &     53.3s &    5.1s (11.1x) &   2.5s (21.1x) \\
5D-U-10M &   383.2s &    346.2s &   19.7s (19.4x) &  17.3s (20.0x) \\
5D-V-10M &   116.1s &    100.9s &    8.8s (13.1x) &   8.8s (11.4x) \\
7D-U-10M &  2365.8s &   2172.9s &  100.2s (23.6x) &  96.4s (22.5x) \\
7D-V-10M &   160.3s &    132.8s &   14.7s (10.9x) &   17.1s (7.8x) \\
10D-H-1M &    24.7s &     19.2s &    2.1s (12.0x) &   1.7s (11.1x) \\
16D-C-4M &   419.6s &    467.0s &   21.1s (19.9x) &  28.5s (16.4x) \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/knn_consolidated-object.tex <==
\begin{tabular}{@{}l@{\hskip1.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip1.5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &       B1 &       B2 &        BDL &             B1 &             B2 &              BDL \\
\midrule
2D-U-10M &    34.9s &    11.9s &    64.5s &   0.6s (57.2x) &   0.3s (40.3x) &   1.5s (43.1x) \\
2D-V-10M &    37.2s &    12.7s &    67.0s &   0.7s (57.0x) &   0.3s (40.7x) &   1.5s (43.7x) \\
5D-U-10M &   302.3s &   178.0s &   339.4s &   6.3s (47.6x) &   3.5s (51.4x) &   8.6s (39.4x) \\
5D-V-10M &   109.5s &    64.1s &   145.8s &   2.1s (51.1x) &   1.2s (52.7x) &   3.2s (46.1x) \\
7D-U-10M &  1520.0s &  1239.4s &  1621.6s &  44.3s (34.3x) &  34.1s (36.4x) &  52.9s (30.7x) \\
7D-V-10M &   133.6s &    86.3s &   173.1s &   2.8s (48.1x) &   1.7s (50.7x) &   4.0s (43.8x) \\
10D-H-1M &     5.3s &     5.5s &    11.9s &   0.1s (54.5x) &   0.1s (50.5x) &   0.3s (45.8x) \\
16D-C-4M &   464.4s &   612.2s &   468.3s &  16.5s (28.1x) &  16.1s (38.1x) &  17.3s (27.1x) \\
3D-C-321M & -- & -- & -- & -- & -- & 15.6s \\
\bottomrule
\end{tabular}


==> batch-kdtree/data/knn_consolidated-spatial.tex <==
\begin{tabular}{@{}l@{\hskip1.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip2.5pt}l@{\hskip1.5pt}l@{}}
\toprule
{} & \multicolumn{3}{@{}l}{1} & \multicolumn{3}{@{}l}{36h} \\
{} &       B1 &       B2 &        BDL &             B1 &             B2 &              BDL \\
\midrule
2D-U-10M &    33.6s &    13.0s &    69.9s &   0.6s (55.6x) &   0.3s (40.0x) &   1.6s (44.9x) \\
2D-V-10M &    35.7s &    13.5s &    72.7s &   0.6s (56.8x) &   0.3s (39.5x) &   1.6s (44.9x) \\
5D-U-10M &   348.8s &   216.7s &   503.1s &   6.7s (52.2x) &   4.0s (54.1x) &   9.6s (52.2x) \\
5D-V-10M &   103.1s &    65.2s &   174.2s &   2.0s (52.8x) &   1.4s (45.4x) &   3.5s (49.5x) \\
7D-U-10M &  2142.0s &  1494.0s &  2804.0s &  45.5s (47.1x) &  36.7s (40.7x) &  57.3s (48.9x) \\
7D-V-10M &   116.9s &    81.3s &   203.1s &   2.3s (50.5x) &   1.7s (48.0x) &   4.1s (49.3x) \\
10D-H-1M &     5.7s &     4.7s &    15.5s &   0.1s (54.6x) &   0.1s (45.2x) &   0.3s (47.3x) \\
16D-C-4M &   606.7s &   557.0s &   623.4s &  19.9s (30.5x) &  11.9s (47.0x) &  20.4s (30.5x) \\
3D-C-321M & -- & -- & -- & -- & -- & 17.4s \\
\bottomrule
\end{tabular}


==> batch-kdtree/pseudocode/bhl-construct.tex <==
\begin{algorithm}
\caption{Parallel $kd$-Tree Construction}\label{alg:bhl-construct}
% 
\hspace*{\algorithmicindent} \textbf{Input}: Point Set $P$ \\
\hspace*{\algorithmicindent} \textbf{Output}: \kdtree{} over $P$, laid out with a binary-heap layout on a contiguous memory space of size $2|P| - 1$.
\begin{algorithmic}[1]
\Procedure{\buildbhl{}}{$P$}
    \State Allocate $2|P| - 1$ nodes in contiguous memory. The tree nodes will be laid out in this space.
    \State \textsc{\buildbhlrecursive{}($P$, 0, 0)}
\EndProcedure
\Procedure{\buildbhlrecursive{}}{$Q$, $idx$, $c$}
\Statex $idx$: current node index
\Statex $c$: current dimension to split on
\State If we hit the base case $|Q| = 1$, then we construct a leaf node to represent $Q$ at the current index and return.
\State Otherwise, perform a parallel median partition on $Q$ in dimension $c$. Then, place an internal node at the current index to represent this split.
\State Compute $med = |Q|/2$. Then, construct the left and right subtrees in parallel with
\begin{align*}
&\textsc{\buildbhlrecursive{}($Q[:|Q|/2]$, $2idx+1$, $(c+1)\mod{d}$)}\\
&\textsc{\buildbhlrecursive{}($Q[|Q|/2:]$, $2idx+2$, $(c+1)\mod{d}$)}
\end{align*} 
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> batch-kdtree/pseudocode/log-knn.tex <==
\begin{algorithm}[!t]
\caption{Data-Parallel \ourtree{} \knn{}}\label{alg:log-knn}
% 
\hspace*{\algorithmicindent} \textbf{Input}: Point Set $S$ \\
\hspace*{\algorithmicindent} \textbf{Output}: An array of arrays of the $k$ nearest neighbors of each point in $S$.
\begin{algorithmic}[1]
\Procedure{\knnlog{}}{$S$}
\State Allocate a \knn{} buffer for each of the points in $S$.
\State For each nonempty tree in the \ourtree{}, in serial, call the parallel subroutine \textsc{\knnserial($S$)} on the individual tree, passing the same set of buffers.
\State After all of the individual \textsc{\knnserial{}} calls are complete, gather and return the results from the \knn{} buffers.
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> batch-kdtree/pseudocode/single-knn.tex <==
\begin{algorithm}
\caption{Data-Parallel $kd$-Tree $k$-NN}\label{alg:single-knn}
% 
\hspace*{\algorithmicindent} \textbf{Input}: Point Set $P$, int $k$ \\
\hspace*{\algorithmicindent} \textbf{Output}: An array of arrays of the $k$ nearest neighbors of each point in $P$.
\begin{algorithmic}[1]
\Procedure{knn}{$P$}
    \State Allocate a $k$-NN buffer $buf_p$ and Call \textsc{KnnSinglePoint(0, $p$, $k$, $buf_p$)} in parallel over all $p\in P$.
\EndProcedure
\Procedure{knnSinglePoint}{$idx$, $p$, $k$, $buf$}
\State If the current node is a leaf, add all points in the leaf to the $buf_p$ and return.
\State Otherwise, recurse on the child $c$ that $p$ falls within based on the current splitting plane.
\State After the recursive call returns, if $buf_p$ does not yet have $k$ points, simply add all the points in the subtree of $c$'s sibling, $s$.
\State On the other hand, if $buf_p$ has $k$ points, obtain the current radius estimate and call \textsc{knnPrune} on $s$.
\EndProcedure
\Procedure{knnPrune}{$idx$, $p$, $k$, $buf$, $rad$}
\State Call the box centered on $p$ with side lengths $2\cdot rad$ the query box.
\State Compute the box intersection of query box with the bounding box of the current node $idx$.
\State If the boxes are disjoint, return immediately - there are no potential closer neighbors in the subtree.
\State If the query box entirely contains the bounding box, add all the points in the subtree to $buf$ - any of these points could potentially be a closer neighbor.
\State If the boxes otherwise overlap, recurse on the left and right children of $idx$ if it is an internal node. Otherwise, add all of its points to $buf$.
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> batch-kdtree/sections/analysis.tex <==
\section{Work-Span Analysis}
\subsection{Individual Tree Routines}
\begin{itemize}
    \item Construction
    \begin{itemize}
        \item CO
        \item BHL
    \end{itemize}
    \item Insert
    \begin{itemize}
        \item Baseline 1
        \item Baseline 2
    \end{itemize}
    \item Delete
    \begin{itemize}
        \item Baseline 1
        \item Baseline 2
    \end{itemize}
    \item $k$-NN
    \item Dual $k$-NN
\end{itemize}

\subsection{Log-Tree Routines}
\begin{itemize}
    \item Construction
    \item Insert
    \item Delete
    \item $k$-NN
    \item Dual $k$-NN
\end{itemize}

==> batch-kdtree/sections/conclusion.tex <==
\section{Conclusion}
F

% Future work includes exploring further splitting heuristics, vectorized operations and other performance engineering, and supporting more query types.

==> batch-kdtree/sections/experiments/plot-insert-batch.tex <==
\begin{figure*}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/batch/insert_2D-V-10M.pdf}
        \caption{Insertions on 2D-V-10M.}
        \label{fig:batch-insert-2dv}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/batch/insert_7D-U-10M.pdf}
        \caption{Insertions on 7D-U-10M.}
        \label{fig:batch-insert-7du}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/batch/delete_2D-V-10M.pdf}
        \caption{Deletions on 2D-V-10M.}
        \label{fig:batch-delete-2dv}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/batch/delete_7D-U-10M.pdf}
        \caption{Deletions on 7D-U-10M.}
        \label{fig:batch-delete-7du}
    \end{subfigure}
    \caption{Plot of throughput (operations per second) of batch insertions and batch deletions vs. batch size for the 2D-V-10M and 7D-U-10M data sets.}
\end{figure*}

==> batch-kdtree/sections/experiments/plot-mixed-ops.tex <==
\begin{figure*}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/vary_k/TPUT_k-NN_2D-V-10M.pdf}
        \caption{\knn{} on 2D-V-10M.}
        \label{fig:varyk-knn-2dv}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{batch-kdtree/graphs/vary_k/TPUT_k-NN_7D-U-10M.pdf}
        \caption{\knn{} on 7D-U-10M.}
        \label{fig:varyk-knn-7du}
    \end{subfigure}
    \caption{Plots of \knn{} throughput (operations per second) vs. $k$ using all 36h cores with hyperthreading,
    for the 2D-V-10M and 7D-U-10M data sets.}
\end{figure*}


==> batch-kdtree/sections/experiments/table-construction.tex <==
\begin{table*}
\inputsubtable{batch-kdtree/data/construction_100-object}{Object median.}{tab:construction-object}
\inputsubtable{batch-kdtree/data/construction_100-spatial}{Spatial median.}{tab:construction-spatial}
\caption{Construction times (seconds) for a single thread (1) and 36 cores with hyper-threading (36h). The self-relative speedup for each implementation and data set is shown in parentheses.}
\end{table*}

==> batch-kdtree/sections/experiments/table-deletion.tex <==
\begin{table*}
\inputsubtable{batch-kdtree/data/delete_10-object}{Object median.}{tab:delete-object}
\inputsubtable{batch-kdtree/data/delete_10-spatial}{Spatial median.}{tab:delete-spatial}
\caption{Batch deletion times (seconds) for a single thread (1) and 36 cores with hyper-threading (36h). The self-relative speedup for each implementation and dataset is shown in parentheses.
We delete batches of 10\% of each dataset, starting from a full tree until the entire dataset has been deleted.}
\end{table*}


==> batch-kdtree/sections/experiments/table-insertion.tex <==
\begin{table*}
\inputsubtable{batch-kdtree/data/insert_10-object}{Object median.}{tab:insert-object}
\inputsubtable{batch-kdtree/data/insert_10-spatial}{Spatial median.}{tab:insert-spatial}
\caption{
Batch insertion times (seconds) for a single thread (1) and 36 cores with hyper-threading (36h). The self-relative speedup for each implementation and data set is shown in parentheses.
We insert batches of 10\% of each data set, starting from an empty tree until the entire data set has been inserted.}
\end{table*}


==> batch-kdtree/sections/experiments/table-knn.tex <==
\begin{table*}
\inputsubtable{batch-kdtree/data/knn_consolidated-object}{Object median.}{tab:knn-object}
\inputsubtable{batch-kdtree/data/knn_consolidated-spatial}{Spatial median.}{tab:knn-spatial}
\caption{
\knn{} times (seconds) for a single thread (1) and 36 cores with hyper-threading (36h). The self-relative speedup for each implementation and data set is shown in parentheses.
We use 100\% of dataset except for 3D-C-321M, which was run with 10\% of the data set because the full \knn{} results could not fit in memory. }
\end{table*}


==> batch-kdtree/sections/implementations.tex <==
\section{Implementation and Optimizations}
In this section, we describe implementation details and optimizations that we developed to speed up the \ourtree{} in practice.

\subsection{Parallel Bloom Filter}
The bloom filter is a probabilistic data structure for testing set membership, 
which can give false positive matches but no false negative matches~\cite{bloom1970}.
When erasing a batch of points from the \ourtree{}, we need to
potentially search for every point to be deleted within every individual underlying \kdtree{}.
To mitigate this overhead, we use a bloom filter to prefilter points to be erased from each individual \kdtree{} that definitely are not contained within it.
Specifically, we implemented a parallel bloom filter and added one to each individual \kdtree{} within the \ourtree{} to track the points in that individual \kdtree{}. Before erasing an input batch from each individual \kdtree{}, we filter the batch with that \kdtree{}'s bloom filter.
This optimization adds some overhead to the construction and insertion subroutines, but provides significant benefits for the delete subroutine. To mitigate some of this overhead, we construct the bloom filters only when they are needed, rather than during construction.

\subsection{Data-Parallel \knn{} Structure}
We tested three different variants of the data-parallel \knn{} search in order to determine the best parallelization scheme. Each scheme consists of 2 nested for loops; one over the input points and one over the individual \kdtrees{}. In the first variant, the outer loop is over the points and the inner loop is over the \kdtrees{}. We only parallelize the outer loop, so we perform a \knn{} search over all the trees for each point in parallel.
% \julian{I don't understand the difference between the first and second variant. elaborate on loop orders} 
In the second variant, we switch the loop order, so the outer loop is over the \kdtrees{} and the inner loop is over points. We parallelize both the inner and outer loops, so we perform a \knn{} search over each of the trees in a data-parallel fashion (i.e., search for the nearest neighbors of each point in parallel), but we also parallelize over the trees. In this case, because our \knn{} buffer is not thread-safe, for each point we have to allocate a separate buffer for each tree and combine the results at the end, which adds some extra overhead. In the third variant, described in Section~\ref{alg:dpknn}, the outer loop is over the \kdtrees{} and the inner loop is over points, but in contrast to the second scheme, we only parallelize the inner loop over points. So, we perform a data-parallel \knn{} over each of the individual \kdtrees{}, one at a time. We found that the second scheme gives the most parallelism, but the third scheme has the fastest end-to-end running time, both serially and in parallel. This is due to better cache locality of the third method---each tree is completely processed before moving on to the next one. One other optimization we used in this third scheme was to process the underlying trees in order from largest to smallest. We experimentally found that the data-parallel \knn{} search scaled better on large trees, and so this gave better radius estimates earlier (as opposed to processing the trees from smallest to largest). 

%\todo{can also discuss different pruning strategies we tried, but seems irrelevant}

% \subsection{Dual-Tree \knn{}} \julian{I think we can remove this section. we can just say in the experiments section that we tried implementing various versions of a parallel dual-tree \knn{} but it was slower in practice due to lower parallelism.} We also implemented several variants of a parallel dual-tree \knn{}~\cite{curtin-dualtree, knn-original-dualtree, curtin-faster-dualtree, esmt}. This approach was theoretically very well-suited to our logarithmic tree structure because we have several individual \kdtrees{} over which we would like to perform a $k$-NN search for the same set of query points. So, to implement this search, we simply have to build a single $kd$-tree over the set of query points. Then, we perform a parallel dual-knn search on each of the underlying trees in order, one at a time. As seen in the experiments (Section~\ref{exp:dualtree-knn}), this did in fact reduce the total amount of work (measured by runtime with a single core) performed by the \knn{} search, as opposed to our other implementations. However, we were not able to derive as much parallelism with this approach and it was slower in parallel. We also experimented with different approaches, such as parallelizing the dual-tree search across all the underlying trees rather than processing them one at a time, but this only increased work and decreased parallelism due to synchronization overheads.

% When implementing the parallel dual-tree \knn{}, we implemented and benchmarked three different variants. In the scheme presented in Section~\ref{alg:log-dknn}, we build a single query \kdtree{} over all of the input points, and then perform a parallel dual-tree \knn{} search on each of the underlying trees one at a time. However, we can also parallelize this search, performing the dual-tree \knn{} on all the trees in parallel. This requires some modifications to our data structures. First off, because the \knn{} buffers are not thread-safe, we have to allocate separate \knn{} buffers for each individual tree and combine the results to a single set of $k$ nearest neighbors at the end. In addition, in the dual-tree \knn{} algorithm~\cite{curtin-dualtree, knn-original-dualtree, curtin-faster-dualtree, esmt}, every node in the query tree tracks a radius field representing the current radius of the \knn{} search of all points in the subtree rooted at that node. We can enable parallelism across the individual dual-tree \knn searches either by making this field atomic, so that all the searches share a single radius estimate, or by making this field an array, so that each search has a separate radius estimate. We found that overall, parallelizing across the trees in this manner led to decreased performance and scalability, as seen in Section~\ref{exp:dualtree-knn}.

\subsection{Parallel Splitting Heuristic} \label{sec:splitting-heuristic}
We implemented two different splitting heuristics for our \kdtrees{}: splitting by object median and splitting by spatial median. Object median refers to a true median---at each split, we split around the median of the coordinates of the points in that dimension. On the other hand, for spatial median, we compute the average of the minimum and maximum of the coordinates of the points in the current dimension and use this as the splitting hyperplane. 
The spatial median is faster to compute, but leads to potentially less balanced trees as it is not strictly splitting the points in half at every level. 
We implement the object median with a parallel in-place sort \cite{jaja, parlaylib} and we implement the spatial median in two steps. First, we perform two parallel prefix sums, using $\min()$, $\max()$ as the predicate functions, to compute the minimum and maximum of the values, respectively. Then, we compute the spatial median as the average of these values and perform a parallel partition around this value.
% \julian{is this a parallel prefix sum followed by a a parallel partition. elaborate on the parallel primitives used.}

% \subsection{Buffer Region}\yiqiu{Maybe we can remove this optmization as it did not work as suggested by the description below}\rahul{yeah i'll probably remove when cutting tomorrow}
% We tested a simple linear array to serve as the buffer region, rather than using a small \kdtree{}, but this severely impacted \knn{} performance, as the \knn{} work on a linear array scales as the product of the size of the array and the size of the query point set. It did, however, provide minor improvements in update speeds. Ultimately, this was not enough to offset the impact on \knn{} performance.

\subsection{Coarsening}
We introduced a number of optimizations that were controlled by tunable parameters in our implementation. One key optimization was the coarsening of leaves, in which we let each leaf node represent up to 16 points rather than 1. This reduces the amount of space needed for node pointers and also improves cache locality when traversing the tree, as the points in a leaf node are stored contiguously.
A second key optimization was the coarsening of the serial base cases of our algorithms, in which we switch from a parallel algorithm to a serial version for recursive cases involving subtrees with less than 1000 points in order to mitigate the overhead of spawning new threads. A third parameter was the buffer tree size, which we set to 1024.
% \julian{specify what the threshold was}

% \julian{specify the buffer size}


%\julian{not sure what this means. we could remove it} Through all these implementations, we make careful use of move semantics to minimize data movement and maximize performance.

==> batch-kdtree/sections/introduction.tex <==
\section{Introduction}

Nearest neighbor search is used in a wide range of applications, such as in databases, machine learning, data compression, and cluster analysis. One popular data structure for supporting $k$-nearest neighbor (\knn{}) search in low dimensional spatial data is the \kdtree{}, originally developed by Bentley~\cite{bentley1975}, as it efficiently builds a recursive spatial partition over point sets.

There has been a significant body of work (e.g.,~\cite{bentley1975, bentley-logarithmic-1, bentley-logarithmic-2, pankaj-co, agarwal2016parallel, curtin-faster-dualtree,wehr2018gpu, zellmann2019binned, bkd}) devoted to developing better \kdtree{} variants, both in terms of parallelization and spatial heuristics. However, none of these approaches tackle the problem of parallelizing batched updates, which is important given that many real-world data sets are being frequently updated. In particular, in a scenario  where the set of points is being updated in parallel, existing approaches either become imbalanced or require full rebuilds over the new point set. 
The upper tree in Figure~\ref{fig:baselines} shows the baseline approach that simply rebuilds the \kdtree{} on every insert and delete, maintaining perfect spatial balance but adding overhead to the update operations. On the other hand, the lower tree in Figure~\ref{fig:baselines} shows the other baseline approach, which never rebuilds and instead only inserts points into the existing spatial partition and marks deleted points as tombstones. This gives fast updates at the cost of potentially skewed spatial partitions.

 \begin{figure}[!t]
     \centering
     \includegraphics[width=0.32\textwidth,trim={0 140 250 0},clip]{batch-kdtree/figures/baselines.pdf}
     \caption{Difference in baseline update strategies when the 2-dimensional points $(5,5)$ and $(7,7)$ are inserted into a spatial-median \kdtree{} initially constructed on the points $(1,1)$ and $(3,3)$. The internal nodes are labeled with the splitting dimension and the coordinate of the split in that dimension. Baseline 1 rebuilds the \kdtree{} on every insertion and deletion, while baseline 2 does not rebuild the tree and instead inserts points into the existing spatial partition.}
     \label{fig:baselines}
 \end{figure}
% In addition to this data structure, we also develop two baseline implementations of \kdtrees{} that support parallel batched updates to evaluate our data structure against. The two baselines represent two different design decisions that could be made to implement batch-dynamic updates on \kdtrees{}. The first baseline implementation simply rebuilds the structure on every insert and delete. This structure maintains perfect spatial balance but adds overhead to the update operations. The second baseline never rebuilds the tree but only inserts points into the existing spatial partition. This achieves very fast updates at the cost of potentially skewed spatial partitions.

Procopiuc \etal{}~\cite{bkd} tackled the problem of a dynamically changing point set with their Bkd-Tree, a data structure for maintaining spatial balance in the face of batched updates. 
However, it was developed for the external memory case and is not parallel. Similarly, Agarwal \etal{}~\cite{pankaj-co} developed a dynamic cache-oblivious \kdtree{}, but it was not parallel and did not support batch-dynamic operations.

We adapt these approaches and develop \ourtree{}, a new parallel, in-memory \kdtree{}-based data structure that supports batch-dynamic operations (in particular, batch construction, insertion, and deletion) as well as exact \knn{} queries. 
\ourtree{}s consist of a set of exponentially growing \kdtrees{} and perform batched updates in parallel. This structure can be seen in Figure~\ref{fig:logmethod}. Just as in the Bkd-tree and cache-oblivious tree, our tree structure consists of a small buffer region followed by exponentially growing static \kdtrees{}. Inserts are performed by rebuilding the minimum number of trees necessary to maintain fully constructed static trees. Deletes are performed on the underlying trees, and we rebuild the trees whenever they drop to below half of their original capacity. Our use of parallelism, batched updates, and our approach to maintaining balance after deletion are all distinct from the previous trees that we draw inspiration from. We show that given a \ourtree{} with $n$ points, each batch of $B$ updates takes $O(B\log^2{(n+B)})$ amortized work and $O(\log{(n+B)}\log\log{(n+B)})$ depth (parallel time). As part of our work, we develop, to our knowledge, the first parallel algorithm for the construction of cache-oblivious \kdtrees{}. 
Our construction algorithm takes $O(n\log n)$ work and $O(\log n\log\log n)$ depth. 
In addition, we implement parallel bloom filters to improve the performance of batch updates in practice. We also present a cache-efficient method for performing \knn{} queries in \ourtree{}.


We show theoretically that \ourtree{}s have strong asymptotic bounds on the work and depth of its operations. 

% \input{batch-kdtree/sections/introduction/fig-log-method}

We experimentally evaluate \ourtree{}s by designing a set of benchmarks to compare its performance against the two baseline approaches described above, which we implemented using similar optimizations. First, we perform scalability tests for each of the four main operations, construction, batch insertion, batch deletion, and \knn{} in order to evaluate the scalability of our data structure on many cores. On a 36-core machine with two-way hyper-threading, we find that our data structure achieves self-relative speedups of up to $35.4\times$ ($30.0\times$ on average) for construction, up to $35.0\times$ ($28.3\times$ on average) for batch insertion, up to $33.1\times$ ($28.5\times$ on average) for batch deletion, and up to $46.1\times$ ($40.0\times$ on average) for full \knn{}. The largest dataset we test consists of 321 million 3-dimensional points.
Then, we design a set of benchmarks that perform a mixed set of updates and queries in order to better understand the performance of \ourtree{}s in realistic scenarios. 
We find that, when faced with a mixed set of batch operations, \ourtree{}s consistently outperforms the two baselines and presents the best option for such a mixed dynamic setting.
% The contributions of this paper are as follows.
% \begin{enumerate}
%     \item \ourtree{}, a new parallel, batch-dynamic \kdtree{} with polylogarithmic depth.\miss{work bounds}
%     \item A new parallel construction algorithm for cache-oblivious \kdtree{} with a vEB layout~\cite{pankaj-co} that is work-efficient ($O(N\log{N})$ work) and has polylogarithmic depth ($O(\log{N}\log\log{N})$).
%     \item An extensive experimental evaluation that demonstrates that \ourtree{}s achieve strong parallel speedups over its single-threaded running time, and outperforms both baselines in the case of mixed updates and queries.
% \end{enumerate}
% Our source code implementing \ourtree{}s is publicly available at \url{https://github.com/rahulyesantharao/batch-dynamic-kdtree}.


==> batch-kdtree/sections/introduction/fig-baselines.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.32\textwidth,trim={0 140 250 0},clip]{batch-kdtree/figures/baselines.pdf}
    \caption{Difference in baseline update strategies when the 2-dimensional points $(5,5)$ and $(7,7)$ are inserted into a spatial-median \kdtree{} initially constructed on the points $(1,1)$ and $(3,3)$. The internal nodes are labeled with the splitting dimension and the coordinate of the split in that dimension. Baseline 1 rebuilds the \kdtree{} on every insertion and deletion, while baseline 2 does not rebuild the tree and instead inserts points into the existing spatial partition.} \label{fig:baselines}
\end{figure}


==> batch-kdtree/sections/introduction/fig-log-method.tex <==
 \begin{figure}[!t]
     \centering
     \includegraphics[width=0.4\textwidth,trim={0 140 220 0}]{batch-kdtree/figures/logtree.pdf}
     \caption{Logarithmic method used in \ourtree{}, with $N_s$ underlying static \kdtrees{} and a buffer \kdtree{} of size $X$. }
     \label{fig:logmethod}
 \end{figure}
 

==> batch-kdtree/sections/preliminaries.tex <==
% \section{Preliminaries}

% \subsection{\kdtree{}}
\myparagraph{\kdtree{}}
The \kdtree{}, first proposed by Bentley~\cite{bentley1975}, is a binary tree data structure that arranges and holds spatial data to speed up spatial queries. Given a set $P$ of $n$ $d$-dimensional points, the \kdtree{} is a balanced binary tree where each node represents a bounding box of a subset of the input points. The root node represents all of the points (and thus the tightest bounding box that includes all the points in $P$). Each non-leaf node holds a splitting dimension and splitting value that splits its bounding box into two halves using an axis-aligned hyperplane in the splitting dimension. Each child node represents the points in one of the two halves.
This recursive splitting stops when the nodes hold some small constant number of points---these nodes are the leaves and directly represent the points.

% \subsubsection{\knn{} Search using the \kdtree{}}\label{prelim-knn}
\myparagraph{\knn{} Search using the \kdtree{}}
Given a query coordinate $q$, a \knn{} query finds the $k$ nearest neighbors of $q$
amongst elements of the \kdtree{} by performing a pruned search on the tree~\cite{friedman1977-kdtree-nn}. The canonical approach is to traverse the tree while inserting points in the current node into a buffer that maintains only the
$k$ nearest neighbors encountered so far. Then, entire subtrees can be pruned during the traversal based on the distance of the $k$'th nearest neighbor found so far.

% \subsubsection{Dual-Tree \knn{}}
% \myparagraph{Dual-Tree \knn{}} Besides the canonical approach explained above, there has been a lot of prior work on ``dual-tree" approaches~\cite{curtin-dualtree, curtin-faster-dualtree, knn-original-dualtree, esmt}, which provide speedups on serial batched \knn{} queries. In particular, the dual-tree approach involves building a second \kdtree{} over the set of query points, and then exploring the two trees simultaneously in order to exploit the spatial partitioning provided by the \kdtree{} structure. We parallelized and tested this dual-tree approach in our work.

% \subsection{Batch-Dynamic Data Structures}
% \myparagraph{Batch-Dynamic Data Structures}
% The concept of a parallel batch-dynamic data structure has become popular in recent years~\cite{WangY0S21,dhulipala2021parallel} as an important paradigm due to the availability of large (dynamic) datasets undergoing rapid changes. The idea is to batch together operations of a single type and perform them as a single batched update, rather than one at a time. This approach offers two benefits. First, from a usability perspective, it is often the case (especially in applications with a lot of data) that operations on a data structure can be grouped into phases or batches of a single type, so this restriction in the usage of the data structure does not significantly limit the usefulness of the data structure. Secondly, from a performance perspective, batching together operations of a single type allows us to group together the involved work and derive significantly more parallelism than otherwise might have been possible (while also avoiding the concurrency issues that might arise with batching together operations of varying types).

% \subsection{Baselines}\label{sec:baselines}
% \myparagraph{Baselines}
% In order to benchmark and test the performance of \ourtree{}s, we implement two parallel baseline \kdtrees{} that use opposite strategies for providing batch-dynamism. In particular, the first baseline \kdtree{} simply rebuilds the tree after every batch insertion and batch deletion. With this approach, the tree is able to maintain a fully balanced structure in the face of a dynamically changing dataset, enabling consistently high performance for \knn{} queries. This comes at the cost of reduced performance for updates. The second baseline \kdtree{} never rebuilds the tree and simply maintains the initial spatial partition, inserting points into and deleting points from the existing structure. This allows for extremely fast batch insertions and deletions, but could potentially lead to a skewed structure and cause reduced \knn{} performance. The difference between these two baselines is graphically demonstrated in Figure~\ref{fig:baselines}. We demonstrate experimentally that \logtree{} achieves a balanced tradeoff between these two baseline options for batch-dynamic parallel \kdtrees{} on which we are performing \knn{} queries. It outperforms both in the dynamic setting where \knn{} queries and batched updates are all being used.

% \subsection{Logarithmic Method}\label{prelim-log-method}
% \myparagraph{Logarithmic Method}
% The logarithmic method~\cite{bentley-logarithmic-1, bentley-logarithmic-2} for converting static data structures into dynamic ones is a very general idea. At a high level, the idea is to partition the static data structure into multiple structures with exponentially growing sizes (powers of 2). Then, inserts are performed by only rebuilding the smallest structure necessary to account for the new points. In the specific case of the \kdtree{}, a set of $N_s$ static \kdtrees{} is allocated, with capacities in the set $[2^{0}, 2^{1},\ldots, 2^{N_s-1}]$, as well as an extra buffer tree with size $2^{0}$. Then, when an insert is performed, the insert cascades up from the buffer tree, rebuilding into the first empty tree with all the points from the lower trees. If desired, the sizes of all of the trees can be multiplied by a buffer size $X$, which is some constant that is tuned for performance. This structure is illustrated in Figure~\ref{fig:logmethod}. In the figure, all of the trees shown are full; one can imagine that the tree with size $2^{3}X$ is empty, so the next insert would cause the buffer and trees 0, 1, and 2 to cascade up to it.

% \subsection{Computational Model}
% \myparagraph{Computational Model}
% We use the standard work-depth model~\cite{clrs, jaja} for multicore algorithms to analyze theoretical efficiency. The \textbf{work} of an algorithm is the total number of operations used and the \textbf{depth} is the length of the longest sequential dependence (i.e., the parallel running time). An algorithm with work $W$ and depth $D$ can be executed on $p$ processors in $W/p + O(D)$ expected time~\cite{BL99}. Our goal is to come up with parallel algorithms that have low work and depth.

% \subsubsection{Parallel Primitives} We use the following parallel primitives in our algorithms.
% \begin{itemize}[topsep=1pt,itemsep=0pt,parsep=0pt,leftmargin=15pt]
%     \item \textbf{Prefix sum} takes as input a sequence of values $[a_1,a_2,\ldots,a_n]$, an associative binary operator $\oplus$, and an identity $i$, and returns the sequence $[i,a_1,(a_1\oplus a_2),...,(a_1\oplus a_2\oplus\cdots\oplus a_{n-1})]$ as well as the overall sum of the elements. Prefix sum can be implemented in $O(n)$ work and $O(\log{n})$ depth~\cite{jaja}.
%     \item \textbf{Partition} takes an array $A$, a predicate function $f$, and a partition value $p$ and outputs a new array such that all the values $a\in A, a<p$ appear before all the values $a\in A, a\ge p$. Partition can be implemented in $O(n)$ work and $O(\log{n})$ depth~\cite{jaja}.
%     \item \textbf{Median partition} takes $n$ elements and a comparator and partitions the elements based on the median value in $O(n)$ work and $O(\log n\log\log n)$ depth~\cite{jaja}. 
% \end{itemize}

% \myparagraph{Parallel Primitives}
% \pack{} takes an array $A$ and a predicate function $f$, and returns a new array containing $a \in A$ for which $f(a)$ is true, in the same order that they appear in $A$.
% \writeMin{} is a priority concurrent write that takes as input two arguments, where the first argument is the location to write to and the second argument is the value to write; on concurrent writes, the resulting value is the smallest value written.


==> batch-kdtree/sections/references.tex <==
% \begin{thebibliography}{00}
% % \bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
% \bibitem{esmt} William B. March, Parikshit Ram, and Alexander G. Gray. 2010. Fast euclidean minimum spanning tree: algorithm, analysis, and applications. In \emph{Proceedings of the 16th ACM SIGKDD international conference on Knowledge discovery and data mining} (\emph{KDD '10}). Association for Computing Machinery, New York, NY, USA, 603–612. DOI:https://doi.org/10.1145/1835804.1835882

% %% related-work (kd-tree and parallel construction)

% \bibitem{bently1975} Bentley, J. L. (1975). Multidimensional binary search trees used for associative searching. Communications of the ACM, 18(9), 509-517.

% \bibitem{shevtsov2007parallelkd} Shevtsov, M., Soupikov, A., & Kapustin, A. (2007, September). Highly parallel fast KD‐tree construction for interactive ray tracing of dynamic scenes. In Computer Graphics Forum (Vol. 26, No. 3, pp. 395-404). Oxford, UK: Blackwell Publishing Ltd.

% \bibitem{agarwal2016parallel} Agarwal, P. K., Fox, K., Munagala, K., & Nath, A. (2016, June). Parallel algorithms for constructing range and nearest-neighbor searching data structures. In Proceedings of the 35th ACM SIGMOD-SIGACT-SIGAI Symposium on Principles of Database Systems (pp. 429-440).

% \bibitem{wehr2018gpu} Wehr, D., & Radkowski, R. (2018). Parallel kd-tree construction on the GPU with an adaptive split and sort strategy. International Journal of Parallel Programming, 46(6), 1139-1156.

% \bibitem{zellmann2019binned} Zellmann, S., Schulze, J. P., & Lang, U. (2019). Binned kd tree construction for sparse volume data on multi-core and GPU systems. IEEE transactions on visualization and computer graphics.

% \bibitem{parlaylib} Guy E. Blelloch, Daniel Anderson, and Laxman Dhulipala. 2020. ParlayLib - A Toolkit for Parallel Algorithms on Shared-Memory Multicore Machines. In Proceedings of the 32nd ACM Symposium on Parallelism in Algorithms and Architectures (SPAA '20). Association for Computing Machinery, New York, NY, USA, 507–509. DOI:https://doi.org/10.1145/3350755.3400254

% %\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
% %\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
% %\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
% %\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
% %\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
% %\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
% \end{thebibliography}

\bibliographystyle{IEEEtran}
\bibliography{refs}

==> batch-kdtree/sections/related-work.tex <==
\section{Related Work}
    Numerous tree data structures for spatial search have been proposed
    in the literature, including the \kdtree{}~\cite{bentley1975},
    quadtree~\cite{finkel1974quad}, ball tree~\cite{omohundro1989five},
    cover tree~\cite{beygelzimer2006cover}, and the R-tree~\cite{guttman1984r}.
    Among them, the \kdtree{} is a well-known data structure proposed by
    Bentley~\cite{bentley1975} in 1975.
    It is simple and yet can handle many types of
    queries efficiently. Bentley showed that the \kdtree{} incurs $O(\log n)$
    time for insertion and deletion of random nodes, and logarithmic average
    query time was observed in practice.
    The data structure has been extensively studied in the parallel setting.
    Shevtsov~\cite{shevtsov2007parallelkd}~\etal{} proposed fast construction
    algorithms for the \kdtree{} for ray tracing, by using binning techniques to distribute
    the workload among parallel processors.
    Agarwal~\cite{agarwal2016parallel}~\etal{} proposed parallel algorithms for
    a series of spatial trees, including the \kdtree{} under the massively parallel
    communication (MPC) model.
    Wehr and Radkowski~\cite{wehr2018gpu} proposed fast sorting-based algorithms for
    constructing \kdtrees{} on the GPU.
    Zellmann~\cite{zellmann2019binned} proposed algorithms for CPUs and GPUs
    for \kdtrees{} used in graphics rendering.


    % Ideas related to the dynamic log-structured tree have been proposed and used in many different scenarios.
    The idea of decomposing a data structure into a logarithmic number of structures
    for the sake of dynamism has been proposed and used in many different scenarios.
    Bentley~\cite{bentley-logarithmic-1, bentley-logarithmic-2} first proposed
    dynamic structures for decomposable search problems.
    Specifically, he proposed general methods for converting static
    data structures into dynamic ones with logarithmic multiplicative overhead in cost,
    using a set of static data structures with size being a power of two.
    Agarwal~\etal~\cite{agarwal2016parallel} designed cache-oblivious
    data structures for orthogonal range searching using ideas from the
    log-structured tree.
    O'Neil~\etal~\cite{oneil1996lsm} proposed the log-structured merge (LSM) tree,
    an efficient file indexing data structure that supports efficient
    dynamic inserts and deletes in systems with multiple storage hierarchies.
    Specifically, batches of updates are cascaded over time, from faster storage
    media to slower ones.
   A parallel version of the LSM tree has been implemented~\cite{parallel-lsm}
    by dividing the key-space independently across cores, and processing it in
    a data-parallel fashion.
    Our work, on the other hand, proposes a parallel batch-dynamic \kdtree{},
    where each batch of updates can be processed efficiently in parallel, while supporting efficient \knn{} queries.
    
    We have recently discovered that, concurrent with our work, Dobson and Blelloch~\cite{dobson2021parallel} developed the zd-tree, a data structure that also supports parallel batch-dynamic updates and \knn{} queries. Their insight is to modify the basic \kdtree{} structure by sorting points based on their Morton ordering and splitting at each level based on a bit in the Morton ordering. 
    For \knn{} queries, they provide a root-based method, which is the traditional top-down \knn{} search algorithm and is what we implement, as well as a leaf-based method, which directly starts from the leaves and searches up for nearest neighbors. The leaf-based method works and is faster when the query points are points in the dataset, as it saves the downward traversal to search for the query points. 
    % This could also
    % be applied to our tree. 
    They prove strong work and depth bounds for construction, batch updates, and \knn{} queries assuming data sets with bounded expansion constant and bounded ratio.  Without these assumptions, however, our bounds would be at least as good as theirs.
    % \julian{They prove work and depth bounds for construction, batch updates, and \knn{} queries assuming data sets with bounded expansion constant and bounded ratio. Without this assumption, their bounds match the bounds we show in this paper. (Need to check if this is true)}
    
    %However, we also observe a number of limitations in their work. 
    %\julian{is this a fundamental limitation of their algorithm? or just something they implemented for convenience?}\rahul{i think the caveat is that without this box, you might have to rebuild the entire tree - i think there's an adversarial case where every insertion causes a tree rebuild} 
    In Dobson and Blelloch's implementation, they optimize \knn{} queries by presorting the query points using the Morton ordering to improve cache locality.
    Their algorithm assumes that there is a maximum bounding box where all future data will fit into, while our algorithm does not make this assumption.
    Their implementation discretizes the \texttt{double} coordinates into 64-bit integers in order to perform Morton sort on them. As a result, they can only use at most $64/d$ bits for each of the $d$ dimensions. 
    Directly extending the implementation to higher dimensions would either lead to larger leaf sizes or using larger-width coordinates for 
    the Morton sort, either of which could add overheads. 
    %On the other hand, our algorithm works directly on the \texttt{double} coordinates, and performs well in higher dimensional datasets as we show in our experiments.
    Their experiments consider only 2D and 3D datasets, while we test on higher dimensional datasets as well. 
    For 2D and 3D datasets, the running times that they report seem to be in the same ballpark as our times (their \knn{} queries for constructing the \knn{} graph are much faster than ours due to the presorting described above), after adjusting for number of processors and dataset sizes, but it would be interesting future work to experimentally compare the codes on the same platform and datasets, including higher-dimensional ones. It would also be interesting to integrate some of their optimizations into our code, and to combine the approaches to build a log-structured version of the zd-tree.


    %, which would incur additional overheads. 
    %\julian{I think that extending to higher dimensions would not be that bad. It would incur a $O(d)$ factor overhead to use larger width coordinates in the sort, but we already incur a $O(d)$ overhead just from reading coordinates with higher dimensions.}\rahul{I agree - but it would be an overhead over the numbers that they report (they're currently saving quite a bit of overhead by just dealing with 64-bit values rather than points like we do)}\yiqiu{I agree the overhead is on the practical side. Theoretically they can use larger integer for higher dimensions}
    %It is unclear whether this approach can be easily extended to higher dimensions in practice, and whether it works well. 
    %On the other hand, our implementation works for any low-dimensional point datasets, for which we show experimental evaluations in the experiment section.


    % \url{https://docs.google.com/document/d/1B5yg7VNPaIk20k2xjthK6fM1j-ge57ok8JtdtkwUSBA/edit?usp=sharing}


==> plots/hull-speedup.tex <==
\begin{table}[]
\small
\begin{tabular}{|l|c|c|}
\hline
\textbf{Implementation} & \textbf{Speedup Range} & \textbf{Average Speedup} \\ \hline
\multicolumn{3}{|c|}{2D Convex Hull}        \\ \hline
RandInc        & 9.58--13.9x  & 12.5x  \\ \hline
QuickHull      & 26.2--31.8x & 29.5x  \\ \hline
DivideConquer  & 39--44.7x & 42.8x  \\ \hline
Sampling       & 9.51--16.8x  & 12.3x  \\ \hline
\multicolumn{3}{|c|}{3D Convex Hull}        \\ \hline
RandInc        & 3.12--11.9x  & 8.04x   \\ \hline
QuickHull      & 3.70--11.5x  & 7.85x   \\ \hline
DivideConquer  & 8.96--22.1x  & 16.6x  \\ \hline
PseudoHull     & 4.03--24.9x  & 11.8x  \\ \hline
Sampling       & 3.09--18.2x  & 10.2x  \\ \hline
\end{tabular}
\caption{Speedup range and average speedup of convex hull implementations on 36 cores with two-way hyper-threading.}\label{table:hull-speedup}
\end{table}


==> plots/hull-vsn.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=2in]{plots/hull-vsn.pdf}
  \caption{Running time versus data size of \textit{quickhull} in $\mathbb{R}^3$.}
  \label{plot:hull-vsn}
\end{figure}


==> plots/seb-speedup.tex <==
\begin{table}[]
\small
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{3}{|c|}{Smallest Enclosing Ball} \\ \hline
\textbf{Implementation}  & \textbf{Speedup Range} & \textbf{Average Speedup} \\ \hline
Welzl           & 1.89x -- 20.6x   & 8.03x   \\ \hline
WelzlMtf        & 6.31x -- 17.9x   & 11.5x  \\ \hline
WelzlMtfPivot   & 10.1x -- 27.1x  & 20x  \\ \hline
Scan            & 18.6x -- 26x  & 21.2x  \\ \hline
Sampling        & 13.9x -- 22.2x  & 16.8x  \\ \hline
\end{tabular}
\caption{Speedup range and average speedup of smallest enclosing ball implementations on 36 cores with two-way hyper-threading.}\label{table:seb-speedup}
\end{table}


==> plots/seb-vsn.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=2in]{plots/seb-vsn.pdf}
  \caption{Running time versus data size of our parallel sampling-based smallest enclosing ball algorithm in $\mathbb{R}^3$.}
  \label{plot:seb-vsn}
\end{figure}


==> sections/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\myparagraph{Convex Hull}
%
The convex hull of a set of points $P$ in $\mathbb{R}^d$
is the smallest convex polyhedron containing $P$ (in this paper, we assume the dimensionality $d$ is a constant).
It is common to represent the convex hull using a set of
\defn{facets}.
The boundary of two facets is a \defn{ridge}.
For example, in $\mathbb{R}^3$,
assuming the points are in general position
(no four points are on the same plane),
each facet is a triangle, and each ridge is a line
that borders two facets (Figure~\ref{fig:defs}(a)).

\begin{figure}
\centering
  \includegraphics[width=0.5\linewidth]{diagrams/defs.pdf}
  \caption{(a) A facet and a ridge of a convex hull in $\mathbb{R}^3$.
  (b) The support of smallest enclosing ball in $\mathbb{R}^2$.
  }\label{fig:defs}
\end{figure}

The randomized incremental algorithm and the quickhull algorithm
are the most widely used algorithms for solving convex hull in practice.
The randomized incremental algorithm for $\mathbb{R}^d$ was
proposed by Clarkson and Shor~\cite{clarkson89random}.
Given a point data set $P$ in $\mathbb{R}^d$,
the randomized incremental algorithm first constructs a $d$-simplex,
a generalization of a tetrahedron in $d$-dimensions as the initial hull.
Then, the algorithm adds the points to the polyhedron in a random order, updating the hull if necessary.
The overall work of the algorithm is $O(n\log n + n^{\lfloor d/2 \rfloor})$ in expectation.

In practice,
the quickhull algorithm~\cite{greenfield1990, barber1996},
another incremental algorithm, is
often used. 
%The quickhull algorithm for 2-dimensional convex hull
%was first introduced by Greenfield~\cite{greenfield1990}.
%Later, quickhull for higher dimensions was discovered by
%Barber~\etal~\cite{barber1996},
%whose algorithm is a variation of randomized incremental algorithm
%for $\mathbb{R}^d$.
The key improvement of the quickhull algorithm is that,
at each time step, rather than processing
a random point, the algorithm processes a point that
is furthest from a facet, which enables the hull to be expanded more quickly.
%Barber~\etal~\cite{barber1996} showed empirically that this approach
%resulted in fewer points processed during the algorithm.
The quickhull algorithm is by far one of the most common
implementations for convex hull due to its simplicity and efficiency~\cite{leomccormack-hull-impl,qhull-hull-impl,quickhull3d-hull-impl,akuukka-hull-impl,karimnaaji-hull-impl,cgal}.
There have also been works that study parallel implementations of
quickhull,
but they are either limited to $\mathbb{R}^2$~\cite{nher2008divide, srikanth2009parallelizing}, or
do not return the exact convex hull for $\mathbb{R}^3$~\cite{stein2012, tzeng2012finding}.

Recently, Blelloch~\etal~\cite{blelloch2020} proposed a new randomized incremental algorithm that is highly parallel in theory. However, the algorithm does not seem to be practical due to numerous data structures required for bookkeeping. Sequential and parallel algorithms based on divide-and-conquer~\cite{preparata1977hull,aggarwal1988parallel,dadoun1989,amato1992parallel} are not known to be practical for $\mathbb{R}^3$ and above, due to the use of complicated subroutines to merge convex hulls. Other approaches, such as the gift-wrapping algorithm~\cite{chand1970gift}, Graham scan~\cite{graham1972}, and Jarvis march~\cite{jarvis1973}, are either not parallel or are limited to solving convex hull in $\mathbb{R}^2$.

\myparagraph{Smallest Enclosing Ball}
The smallest enclosing ball of $P$ in $\mathbb{R}^d$ is the smallest
$d$-sphere containing $P$.
It is well-known that the smallest enclosing
ball is unique and defined by a \defn{support set} of $d+1$ points on the surface of the ball
(Figure~\ref{fig:defs}(b)).

Welzl~\cite{welzl1991disks} showed that by using a randomized incremental algorithm,
the smallest enclosing ball can be computed in $O(n)$ time 
in expectation for constant $d$.
The algorithm iteratively expands the
support set of the ball by adding points in a random order until the ball contains all of the points.
The algorithm was later improved by Gartner~\cite{gartner1999seb}
with practical optimizations for speed and robustness.
Larsson~\etal~\cite{larsson2016} proposed practical parallel algorithms
that uses a new method for expanding the support set, and the implementation works on both CPUs and GPUs.
Later, Blelloch~\etal~\cite{blelloch2016incremental} proposed a
parallel algorithm based on Welzl's algorithm, but without any
implementations.

In this paper, we develop a parallel algorithm that improves upon Larsson~\etal~\cite{larsson2016}'s
algorithm. We also provide the first implementation of Blelloch~\etal~\cite{blelloch2016incremental}'s algorithm.

\input{batch-kdtree/sections/preliminaries}

% \myparagraph{Parallel Primitives}
% \pack{} takes an array $A$ and a predicate function $f$, and returns a new array containing $a \in A$ for which $f(a)$ is true, in the same order that they appear in $A$.
% \writeMin{} is a priority concurrent write that takes as input two arguments, where the first argument is the location to write to and the second argument is the value to write; on concurrent writes, the resulting value is the smallest value written.


==> sections/related.tex <==
\section{Related Work}

\subsection{Convex Hull}

% \julian{the theory discussion was too long, given that we are not submitting to a theory conference. i removed a lot of the text.}\yiqiu{Sounds good!}

\myparagraph{Theory} 
The convex hull problem has been studied extensively in theory. Fast sequential algorithms have been designed over the past several decades~\cite{chand1970gift,graham1972,jarvis1973,shamos1978thesis,preparata1977hull,seidel1981thesis,kirkpatrick1986ultimate,seidel1986,clarkson89random,seidel1991,chazelle1995derandom,chazelle1993optimal,chan1996optimal}. The best known algorithms that are not output-sensitive take $O(n\log n + n^{\lfloor d/2 \rfloor})$ time for $d$ dimensions~\cite{clarkson89random,chazelle1995derandom,seidel1991}. The fastest output-sensitive algorithms take $O(n\log h)$ time for 2 and 3 dimensions and $O(n^2 + h\log n)$ time for higher dimensions~\cite{kirkpatrick1986ultimate,seidel1986,chazelle1995derandom,chan1996optimal}, where $h$ is the number of facets on the convex hull.
% \julian{elaborate here. maybe the bounds for 2/3 dimensions and higher dimensions are different}. \shangdi{$h$ is the size of the output?} \yiqiu{Yes. All fixed}

% The convex hull problem has been studied in both theory and practice,
% and in both the sequential and parallel context.
% Sequentially,
% Chand and Kapur~\cite{chand1970gift} proposed the gift-wrapping algorithm, which
% runs in $O(n^2)$ time and computes any dimensional convex hull.
% Graham~\cite{graham1972} proposed the famous Graham scan algorithm, which takes $O(n\log n)$ time
% for $\mathbb{R}^2$.
% %The algorithm works by sorting the input points based on the angle
% %to a pre-determined facet, after which the points are processed in a linear scan
% %with back-tracking.
% Jarvis~\cite{jarvis1973} proposed the Jarvis march algorithm for $\mathbb{R}^2$, which takes $O(nh)$ where $h$ is the number of vertices on the output
% convex hull.
% Yao~\cite{yao1981hull-lowerbound} proved an $\Omega (n\log n)$ lower bound for
% the convex hull problem.
% In the thesis of Shamos~\cite{shamos1978thesis}, several $O(n\log n)$ time algorithms
% for 2-dimensional convex hull were proposed \julian{are these different than the ones above?}.
% Preparata and Hong~\cite{preparata1977hull} proposed the first sub-quadratic
% algorithm for $\mathbb{R}^3$ taking $O(n\log n)$ time, using recursive divide-and-conquer.
% Seidel~\cite{seidel1981thesis} showed that convex hull in any even dimensions
% can be solved in $O(n \log n + n^{\lfloor d/2 \rfloor} )$ time, which was the first
% significant result for dimensions higher than 3.
% Later, Kirkpatrick and Seidel~\cite{kirkpatrick1986ultimate} proposed an output-sensitive
% algorithm for planar convex hull, which runs in $O(n\log h)$.
% Seidel~\cite{seidel1986} then proposed output-sensitive algorithms for higher dimensional convex hulls using
% the technique called the straightline shelling of polytopes. The algorithm solves
% convex hull of output size $h$ in $O(n^2 + h\log n)$ time for any dimension.
% Clarkson and Shor~\cite{clarkson89random} gave an optimal randomized algorithm
% which takes $O(n\log n)$ expected time for 3 dimensions and
% $O(n^{\lfloor d/2 \rfloor})$ expected time in $d>3$ dimensions.
% Later, the algorithm was derandomized by Chazelle and Matousek~\cite{chazelle1995derandom}.
% Seidel~\cite{seidel1991} proposed a simpler randomized incremental algorithm for $d$-dimensional
% convex hull, which also takes $O(n^{\lfloor d/2 \rfloor})$ expected time.
% Chazelle~\cite{chazelle1993optimal} proposed a deterministic algorithm
% for any dimension $d$, which takes $O(n\log n + n^{\lfloor d/2 \rfloor})$ time \julian{how is this related to the derandomization by Chazelle and Matousek? it seems that the bounds are the same}.
% Later, Chan~\cite{chan1996optimal} proposed output-sensitive $O(n\log h)$-time algorithms
% for 2-dimensional and 3-dimensional convex hull, which use much simpler
% algorithms than previous results.

The convex hull problem has also been studied theoretically in the parallel setting~\cite{atallah1986parallel,chow1980,aggarwal1988parallel,dadoun1989,amato1992parallel,reif1992,amato1994,amato1993nc,blelloch2020,ghouse1991,gupta2003faster}. The best bounds for 2 and 3 dimensions are $O(n\log n)$ work and $O(\log n)$ depth~\cite{atallah1986parallel,reif1992}. For higher dimensions, it can be solved in $O(n\log n + n^{\lfloor d/2 \rfloor})$ work and $O(\log n)$ depth~\cite{amato1994}.
Among output sensitive algorithms, previous work obtain
$O(n \log h)$ work and  $O(\log n)$ depth for 2 dimensions~\cite{ghouse1991} and
$O(n\log h)$ work and $O(\log\log^2 n \log h)$ depth for 3 dimensions~\cite{gupta2003faster}.
%\julian{discuss the best bounds for the problem (output-sensitive, non output-sensitive, different dimensions). there are no bounds listed for $d>3$ below.}\yiqiu{Summarized. The best bound for $d>3$ is added (from~\cite{amato1994}). I left the longer paragraph in the comments}

% \julian{remove all this text after summarizing the bounds above}
% Atallah and Goodrich~\cite{atallah1986parallel} proposed a parallel algorithm for
% 2-dimensional convex hull, which takes $O(n\log n)$ work and $O(\log n)$ depth.
% Chow~\cite{chow1980} showed that 
% 3-dimensional convex hull can be solved with $O(n\log^3 n)$ work and $O(\log^3 n)$ depth.
% Aggarwal~\etal~\cite{aggarwal1988parallel} described a divide-and-conquer algorithm
% for the 3-dimensional convex hull with the same complexity bounds.
% Later, Dadoun and Kirkpatrick~\cite{dadoun1989},
% and Amato and Preparata~\cite{amato1992parallel}
% improved the result, giving algorithms that take $O(n\log^2 n)$ work and $O(\log^2 n)$ depth. Reif and Sen~\cite{reif1992} proposed the first optimal parallel randomized algorithm
% for 3-dimensional convex hull, taking $O(n\log n)$ expected work and $O(\log n)$ depth with high probability \julian{is depth expected or with high probability?}\yiqiu{With high probability. Fixed}.
% The result was later extended to any constant dimension in $O(\log n)$ depth and $O(n\log n + n^{\lfloor d/2 \rfloor})$ work by Amato~\etal~\cite{amato1994} \julian{list the bounds}\yiqiu{Fixed}.
% Amato and Preparata~\cite{amato1993nc} then proposed a deterministic algorithm that
% takes $O((1/\alpha)n^{1+\alpha}\log n)$ work and $O((1/\alpha)\log n)$ depth, for $0<\alpha\leq 1$.
% %takes $O((1/\alpha)\log n)$ time and $O(n^{1+\alpha})$ processors, for $0<\alpha\leq 1$.
% Recently, Blelloch~\etal~\cite{blelloch2020} proposed a parallel randomized
% incremental algorithm that takes $O(n\log n)$ expected work and $O(\log n\log^* n)$
% depth with high probability.
% Ghouse and Goodrich~\cite{ghouse1991} proposed output-sensitive parallel
% algorithms which take $O(n \log h)$ work and  $O(\log n)$ depth in 2 dimensions, and $O(min\{ n \log^2 h, n\log n \})$ work and $O(\log^2 n)$ depth in 3 dimensions.
% Gupta and Sen~\cite{gupta2003faster} proposed an output-sensitive algorithm
% that takes $O(n\log h)$ work and $O(\log\log^2 n \log h)$ depth.

\myparagraph{Implementations}
% \julian{a discussion of how the following CPU papers are different from our work is missing}\yiqiu{Fixed, at end of paragraph}
The convex hull problem has also been widely studied in practice for 2 and 3 dimensions.
Barber~\etal~\cite{barber1996} studied a variant of the randomized incremental
algorithm, widely known as the
quickhull algorithm.
Cintra~\etal~\cite{cintra2004speculative} studied the 2-dimensional randomized
incremental algorithm using speculative parallelism on multiple cores.
Diaz~\etal~\cite{diaz2004parallelizing} parallelized the computation of
2-dimensional convex hull  using divide-and-conquer in distributed memory.
% They studied the implementations in the distributed context using MPI.
Gonzalez~\etal~\cite{gonzalez2006} compared multiple parallel computing paradigms
using parallel algorithms for 2-dimensional convex hull.
Naher and Schmitt~\cite{nher2008divide} explored a parallel divide-and-conquer
approach for the 2-dimensional convex hull, and provide multicore implementations.
Recently, Gamby and Katajainen~\cite{gamby2019, gamby2019bucketing} implemented
and compared multiple 2-dimensional convex hull algorithms on the CPU,
and proposed a bucketing optimization.
The previous works for the CPU are either restricted to solving
2 dimensions, or are not parallel.
% Our work proposes parallel algorithms and implementations for dimensions 2, 3 and above.

Convex hull algorithms have also been widely implemented on GPUs.
Many of them call a sequential CPU implementation as a subroutine,
which can be a scalability bottleneck. 
% Some of them are limited to $\mathbb{R}^2$,
% or may not return the correct results.
Srikanth~\etal~\cite{srikanth2009parallelizing} implemented
the 2-dimensional quickhull algorithm using CUDA.
Gao~\etal~\cite{gao2013} proposed a new algorithm and implementation for
3-dimensional convex hull, based on generating an approximate hull from the
Voronoi diagram, followed by using a star-splaying approach to fix the convex hull.
% Stein~\etal~\cite{stein2012} proposed ``CudaHull'', a GPU algorithm that computes a 3-dimensional polyhedron resembling a convex hull. It is based on the 3-dimensional quickhull algorithm, but corrects conflicting updates by performing additional polyhedron refinements on the CPU. It was pointed out in Gao~\etal's paper~\cite{gao2013} that the algorithm of Stein~\etal~\cite{stein2012} can be non-convex. Tang~\etal~\cite{tang2012} proposed a GPU based heuristic for the general dimension convex hull. It works by by first generating a ``pseudohull'' polyhedron, in which the points are removed, and the convex hull is then computed on the remaining points sequentially on the CPU.
Stein~\etal~\cite{stein2012} and Tang~\etal~\cite{tang2012} proposed
quickhull-related algorithms for heuristics for the GPU, which we have
discussed in Section~\ref{sec:hull}.
Tzeng and Owens~\cite{tzeng2012finding} implemented 2 and 3-dimensional convex hull on the GPU.
Mei~\etal~\cite{mei2018} came up with alternative implementations based on Tzeng and Owens' implementation.
Recently, Masnadi and LaViola~\cite{masnadi2020} came up with a GPU-based implementation using a grid-based culling heuristic.
We did not explicitly compare with GPU implementations, though we evaluated
some of the techniques in the multicore context.
A significant advantage of our multicore approach is that
we are not bottlenecked by
the limited amount of memory on GPUs today. 
We tested our implementations on data sizes
of up to one billion, which is 10 times larger than the largest data set
used in the literature for GPU-based algorithms.
%\julian{on GPUs? or both CPU and GPU?}\yiqiu{It is GPU, I just found a paper on 2d sequential algorithm with 100M data sets (cited). Fixed}

In addition to the implementations above, there are many open-source implementations available online~\cite{qhull-hull-impl, akuukka-hull-impl, cgtools-hull-impl, sinclair-hull-impl, karimnaaji-hull-impl, quickhull3d-hull-impl, leomccormack-hull-impl, cgal, cphstl-hull-impl}.

% \julian{the comparison with CGAL and qhull, and the speedup numbers should go in the experiments section.}\yiqiu{Fixed}
% We compared with CGAL~\cite{cgal} and qhull~\cite{qhull-hull-impl, barber1996}, the two most common sequential baselines on the CPU. because of the unavailability of the code, and that these implementations are limited to $\mathbb{R}^2$. Comparing with the baselines we chose, we achieved a speedup ranging from 5.68x to 1673.33x.

% There also exists other parallel algorithms and implementations. The GPU algorithm by Gao~\etal~\cite{gao2013} relies on computing a 3-dimensional Voronoi diagram, which is complicated and whose implementation is not generally available on the CPU. There are multiple papers focusing on parallelizing the convex hull~\cite{cintra2004speculative,diaz2004parallelizing,gonzalez2006,nher2008divide,gamby2019}, but they are limited to $\mathbb{R}^2$. There are a few papers focusing on pruning interior points, after which the convex hull is expected to be computed on a smaller input~\cite{tang2012,gamby2019bucketing,masnadi2020}. They do not address the parallel computation of the remaining points, which can become a large bottleneck when most of the input points are vertices of the convex hull.

% Recently, Blelloch~\etal~\cite{blelloch2020} proposed a new randomized incremental algorithm that is highly parallel in theory. The algorithm does not seem to be practical at the moment due to numerous book-keeping data structures required. Sequential and parallel algorithms based on divide and conquer~\cite{preparata1977hull,aggarwal1988parallel,dadoun1989,amato1992parallel} are not known to be practical for $\mathbb{R}^3$ and above, due to the use of complicated subroutines to merge two convex hulls. Other approaches, such as gift-wrapping algorithm~\cite{chand1970gift}, Graham scan~\cite{graham1972}, and Jarvis march~\cite{jarvis1973} are either not parallel, or limited to solving convex hull in $\mathbb{R}^2$.

\subsection{Smallest Enclosing Ball}

% \julian{the discussion below sometimes discusses theoretical bounds and sometimes does not. the theory and implementations are mixed. it would be better to organize them into "Theory" and "Implementation" paragraphs (as done in the related work section for convex hull). for theory, cite all the papers but just state the best bounds.}\yiqiu{Sounds good, fixed}

\myparagraph{Theory}
The smallest enclosing ball problem was first discovered by Sylvester in 1857~\cite{sylvester1857question}, and
has been well studied in theory~\cite{elzinga1972,shamos1975closest,megiddo1982,welzl1991disks,kallberg2016,dearing2009,cavaleiro2018faster,blelloch2016incremental}.
The best algorithms for constant dimensions takes $O(n)$ work.
The fastest parallel algorithm takes $O(n)$ expected work and
$O(\log^d n)$ depth with high probability~\cite{blelloch2016incremental}.
Multiple approximate algorithms have also been proposed in the
literature~\cite{nielsen2004approximating,nielsen2009approximating,yildirim2008two,larsson2013fast,aggarwal1988parallel,ding2019}.

\myparagraph{Implementations}
Gartner~\cite{gartner1999seb} proposed optimizations and improved the robustness of
Welzl's algorithm.
Larsson~\etal~\cite{larsson2016} proposed a new practical algorithm called
orthant-scan.
Gartner and Schonherr~\cite{gartner2000} presented a solver that solves the smallest enclosing disc for moderately higher dimensions.
Fischer~\etal~\cite{fischer2003} developed a simple combinatorial algorithm
for high dimensions.
% Our work focuses on constant dimensions, builds on Larsson's algorithm~\cite{larsson2016} and proposes a faster algorithm and implementation.

% The smallest enclosing ball problem was first discovered by Sylvester in 1857~\cite{sylvester1857question},
% and has been a fundamental problem in computational geometry since then.
% It has been well studied in both theory and practice.
% %For 2-dimensional point data sets, the smallest enclosing ball is unique, and is defined by 2 or 3 support points \julian{this is not true if the data set is degenerate (more than 3 points lie on the circle)}\yiqiu{Dropped the description}.
% A brute-force algorithm would inspect all combinations of possible balls.
% Elzinga and Hearn~\cite{elzinga1972} improved the bruteforce method to
% run in $O(n^2)$ time.
% Then, Shamos and Hoey~\cite{shamos1975closest} proposed an $O(n\log n)$ time
% algorithm using the Voronoi diagram.
% Megiddo~\cite{megiddo1982} was the first to break the barrier and propose
% an $O(n)$ time algorithm using linear programming.
% Welzl~\cite{welzl1991disks} proposed an randomized algorithm which takes
% $O(n)$ expected time, and work for any constant number of dimensions.
% %The basic idea is to form the ball incrementally by processing the points, sequentially in random order.
% % The paper also describes a practical optimization and includes experiments.
% %Later, Gartner~\cite{gartner1999seb} proposed the pivoting optimization technique, robust promitives on top of Welzl's algorithm,
% Later, Gartner~\cite{gartner1999seb} proposed a new optimization and improved robustness of Welzl's algorithm, and contributed an implementation for lower dimensions in the CGAL library~\cite{cgal}.
% Gartner and Schonherr~\cite{gartner2000} presented a solver that specializes in
% quadratic programs for geometry, which solves the smallest enclosing disc
% efficiently in practice for moderately higher dimensions.
% Fischer~\etal~\cite{fischer2003} then developed a simple combinatorial algorithm
% for high dimensions.
% Larsson~\etal~\cite{larsson2016} proposed new practical algorithm called
% orthant scan, which computes the smallest enclosing ball for general dimensions
% quickly.
% Kallberg~\etal~\cite{kallberg2016} proposed an external memory algorithm that
% runs in $O(n/b)$ time, where $b$ is the block size.
% \julian{if this is about the ball of balls problem, you can remove it. otherwise it should be merged with the previous discussion}
% Dearing and Zeck~\cite{dearing2009} discussed a dual-algorithm of the smallest
% enclosing ball, which was later improved by Cavaleiro
% and Alizadeh~\cite{cavaleiro2018faster}.
% Later, Blelloch~\etal~\cite{blelloch2016incremental} came up with
% a parallel algorithm for low dimensions that runs in $O(n)$ expected work and
% $O(\log^2 n)$ depth with high probability.

% Multiple approximate algorithms have been proposed in the literature.
% Nielson and Nock~\cite{nielsen2004approximating,nielsen2009approximating} proposed several fast approximation
% algorithms for the problem. 
% % suitable for real-time applications in the practice.
% % Nielson and Nock~\cite{nielsen2009approximating} then proposed two more approximate
% % algorithms and dicussed applications in machine learning.
% Yildirim~\cite{yildirim2008two} proposed two $(1+\epsilon)$-approximation algorithms in $d$ dimension, which takes $O(nd/\epsilon)$ time.
% Larsson and Kallberg~\cite{larsson2013fast} proposed a fast and robust approximate
% algorithm, with a fast parallel implementation.
% Recently, Ding~\cite{ding2019} studied a relaxed version of the problem with
% sublinear running time. \julian{is this sequential or parallel?}\yiqiu{It's sequential}

% Fischer and Gartner~\cite{fischer2004smallest} solved a closely related problem,
% the smallest bounding balls of balls, which generalizes the smallest bounding
% ball of points.
% Recently, Dearing and Cawood~\cite{dearing2020} proposed primal and dual algorithms
% for the smallest enclosing ball of balls in the Euclidean space.

% Our work focuses on the exact smallest enclosing ball problem in constant dimensions. Therefore, we compared with the implementation in CGAL~\cite{cgal}, written by Gartner following the paper~\cite{gartner1999seb}. We achieved a speedup of 88.36x--177.58x. \julian{this comparison should go in the experiments section}

% \subsection{Frameworks for Geometric Processing}
% There are numerous libraries for algorithms in computational geometry,
% but most of them are not designed for parallel processing.
% Libigl~\cite{libigl} is a library that specializes in
% the construction of discrete differential geometry
% operators and finite-element matrices.
% Only some functionalities of Libigl take advantage of
% parallelism.
% CGAL (The Computational Geometry Algorithms Library)~\cite{cgal}
% is a famous library of computational geometry algorithms
% that includes a wide range of packages.
% Batista~\etal~\cite{batista2010} targeted a few important
% algorithms for shared memory parallel processing, whose code
% is hosted in CGAL.
% PMP~\cite{pmp-library}, Cinolib~\cite{cinolib}, and Tetwild~\cite{tetwild} 
% are libraries for processing
% polygonal and polyhedron meshes.
% % Tetwild supports parallel computation
% % using the Intel Implicit SPMD Program Compiler, which
% % according to the authors, reduces the overall running time
% % by an average of $4\%$.
% MatGeom~\cite{matgeom} is a library for geometric computing
% with MATLAB in 2 and 3 dimensions.
% The Problem Based Benchmark Suite~\cite{pbbs}
% is a multicore benchmark suite that includes multiple geometric
% benchmark such as 2-dimensional Delaunay triangulation, Delaunay refinement, and $k$-nearest neighbor search.
% LEDA~\cite{leda} is a standard library of
% data structures and algorithms for combinatorial and geometric processing.
% ArborX~\cite{arborx} is a library for spatial
% search, designed for high performance computing platforms including
% multicore and GPU.

\input{batch-kdtree/sections/related-work}
